UPDESH: Synthesizing Grounded Instruction Tuning Data for 13 Indic Languages

Developing culturally grounded multilingual AI systems remains challenging, particularly for low-resource languages. While synthetic data offers promise, its effectiveness in multilingual and multicultural contexts is underexplored. We investigate bottom-up synthetic data generation using large open-source LLMs (>= 235B parameters) grounded in language-specific Wikipedia content, complementing dominant top-down translation-based approaches from English. We introduce Updesh, a high-quality large-scale synthetic instruction-following dataset comprising 9.5M data points across 13 Indian languages and English, encompassing diverse reasoning and generative tasks. Comprehensive evaluation using automated metrics and 10K human assessments confirms high data quality. Downstream evaluations performed by fine-tuning models on various datasets and assessing performance across 13 diverse multilingual datasets and model comparative evaluations, demonstrate that models trained on Updesh consistently obtain significant improvements on NLU, NLG evaluations. Finally, through ablation studies and cultural evaluations, we show that context-aware, culturally grounded data generation is essential for effective multilingual AI development.

==> content/framework.tex <==
\section{Framework}
Synthetic data is utilized throughout the AI lifecycle, including pre-training, supervised fine-tuning (SFT), reinforcement learning from human feedback (RLHF), and evaluation \citep{viswanathan-etal-2025-synthetic}. Synthetic data generation starts with a small set of human-curated seeds, which is then provided to an LLM to generate instructions, inputs and outputs, followed by filtering for correctness and quality. An alternate approach is to retrieve the relevant datasets and use an LLM to rewrite them into the desired format. The dominant method for producing multilingual synthetic data involves translating English data with Neural Machine Translation systems or Large Language Models (LLMs) for pre-training \citep{doshi-etal-2024-pretraining,khan-etal-2024-indicllmsuite}, Supervised Fine Tuning (SFT) \citep{shaham-etal-2024-multilingual}, and evaluation. However, translation may introduce translation artifacts (referred to as \textit{translationese}) \citep{zhang-toral-2019-effect,vanmassenhove-etal-2021-machine} and yield weaker correlations with human evaluations compared to benchmarks tailored for particular languages and contexts \citep{kreutzer2025dj,wu2025bitterlessonlearned2000}. Recent work has explored bottom-up approaches that rely on grounding and retrieval augmentation, including instruction backtranslation \citep{li2024selfalignment} and instruction back-and-forth translation \citep{nguyen-etal-2024-better}, which generate high-quality synthetic data grounded in web corpora. These methods can potentially demonstrate superior performance compared to traditional translation-based approaches. However, there remains limited exploration of such approaches in multilingual contexts. In this work, our focus is on curating multilingual, multicultural synthetic data for SFT, although our framework can apply to other kinds of multilingual, multicultural synthetic data, including synthetic pre-training data and preference data as well. Below, we describe the key factors to consider when generating this type of data.

\paragraph{Base model capability} Synthetic data is usually generated by prompting large foundation models due to their fluency, ability to follow instructions, and safety guardrails. For generating multilingual, multicultural synthetic data, candidate base models should be evaluated on established multilingual and multicultural benchmarks to determine performance in target languages. If benchmarks for a specific target language are unavailable, evaluation results from related languages or overall multilingual performance can be used as indicators. Some models list supported languages and may include multilingual benchmark results in their release reports, while others do not provide these details. Additional factors to consider when selecting a base model include licensing, cost, and whether models are open-weights or restricted.

\paragraph{Seed data selection} Seed data is typically selected on the basis of factors such as diversity and target task coverage. Additional considerations for multilingual, multicultural seed data collection would include prioritizing tasks with coverage of cultural knowledge, norms, and values, and tasks with more relevance in specific regional and cultural contexts (for example, agriculture).

\paragraph{Data generation strategy} Several data generation strategies can be considered for synthetic data generation, including translation, back-translation, and retrieval-augmented synthetic data generation. Translating high-quality, curated English SFT datasets allows us to carry over critical skills the LLM needs to acquire into the multilingual training data. Back-translation using existing multilingual datasets can enhance diversity. Retrieval-augmented generation from diverse sources can potentially leverage native speaker-authored content to produce synthetic data that includes cultural knowledge and linguistic nuances.

\paragraph{Quality metrics} Synthetic data should be evaluated for correctness and quality before being used in downstream tasks. This may involve both automated assessment and human evaluation by native speakers. Essential quality metrics for multilingual and multicultural synthetic data include:


\begin{itemize}[noitemsep]
     \item \textit{Language correctness}: Is the data in the right language, register, and dialect, or is there confusion with a similar language? \citep{marchisio-etal-2024-understanding}
    \item \textit{Linguistic acceptability}: Does the data sound fluent and natural to a native speaker of the language? \citep{hada-etal-2024-large,hada-etal-2024-metal}
    \item \textit{Cultural appropriateness}: Does the data contain appropriate references to cultural artifacts and knowledge and accurately reflect values and norms?
    \item \textit{Bias and safety}: Does the data amplify stereotypes, contain unsafe content, or culturally inappropriate outputs?
\end{itemize}

\paragraph{Downstream evaluation} The primary objective of generating synthetic data is to improve model performance in real-world applications, making the choice of downstream tasks for evaluations critical. This is particularly challenging given the scarcity of multilingual and multicultural benchmarks. To address this, downstream benchmarks should cover all target languages and, wherever possible, avoid relying on translated datasets originally in English. They should also include diverse tasks, especially when synthetic data spans multiple domains. They should incorporate tests of cultural knowledge, norms, and values. In some cases, new benchmarks aligned with the target task, language, and cultural context may need to be developed to accurately assess the utility of synthetic data. Finally, care must be taken to avoid benchmark contamination in the base model, a common issue with multilingual benchmarks \citep{ahuja2024contaminationreportmultilingualbenchmarks}.

\paragraph{Native speaker consent, involvement and privacy} Multilingual and multicultural synthetic data creation processes should involve native speakers in seed data selection and evaluation when feasible. Informed consent is required to address cultural considerations and data sovereignty according to local regulations. Synthetic data must not contain personally identifiable information derived from seed data or online sources.

==> content/framework_short.tex <==

\section{Design Considerations}
Our framework (\Cref{fig:framework}) addresses synthetic data generation for multilingual and multicultural contexts throughout the AI lifecycle — pre-training, SFT, RLHF, and evaluation \citep{viswanathan-etal-2025-synthetic}. Below, we describe the key factors to consider when generating this type of data. While our focus is on SFT data, these design considerations can generalize to other synthetic data types.

\paragraph{Base model capability \& Seed data selection} Select foundation models based on performance in target languages on multilingual benchmarks. When language-specific benchmarks are unavailable, use related languages or overall multilingual performance as proxies. Other critical aspects to consider include licensing, cost, and model availability (open-weights vs. restricted). For seed data selection, cover diverse sources and tasks, prioritizing tasks containing cultural knowledge, norms, and values relevant to specific regional contexts.

\paragraph{Data generation strategy} Three primary approaches: (i) \textit{Translation} from English SFT datasets to transfer critical skills, though risking translationese artifacts \citep{zhang-toral-2019-effect,vanmassenhove-etal-2021-machine}; (ii) \textit{Back-translation}—using existing unlabeled multilingual datasets through instruction backtranslation \citep{li2024selfalignment} or back-and-forth translation \citep{nguyen-etal-2024-better}; (iii) \textit{Retrieval-augmented generation} —leveraging curated native speaker-authored content from web corpora to capture cultural knowledge and linguistic nuances. Translation-based approaches yield weaker correlations with human judgements than language-specific benchmarks \citep{kreutzer2025dj,wu2025bitterlessonlearned2000}. Bottom-up approaches grounded in web corpora show superior performance \citep{shaham-etal-2024-multilingual,khan-etal-2024-indicllmsuite,doshi-etal-2024-pretraining} but remain underexplored in multilingual contexts.

\paragraph{Quality metrics} Essential dimensions for assessment: \textit{Language correctness}—proper language, register, dialect identification \citep{marchisio-etal-2024-understanding}; \textit{Linguistic acceptability}—native speaker fluency and naturalness \citep{hada-etal-2024-large,hada-etal-2024-metal}; \textit{Cultural appropriateness}—accurate cultural references, values, and norms; \textit{Bias and safety}—absence of stereotypes and culturally inappropriate content \citep{10.1162/COLI.a.14}.

\paragraph{Downstream evaluation} Select benchmarks covering all target languages, avoiding English-translated datasets. Include diverse tasks testing cultural knowledge and values. Address benchmark contamination risks \citep{ahuja2024contaminationreportmultilingualbenchmarks} and develop new benchmarks when necessary.

\paragraph{Native speaker involvement} Engage native speakers in seed selection and evaluation. Ensure informed consent addressing cultural considerations and data sovereignty per local regulations. Exclude personally identifiable information from all sources. 

==> content/results.tex <==
\section{Downstream performance}
% \input{tables/downstream_evaluation}

\begin{table}[H]
\centering
\input{tables/downstream_evaluation}
\end{table}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{evaluation_plots/IFEval.png}
%     \caption{IFEval - English}
%     \label{fig:placeholder}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{evaluation_plots/GlobalMMLU.png}
%     \caption{GlobalMMLU}
%     \label{fig:placeholder}
% \end{figure}




\paragraph{Task-type sensitivity (NLU vs.\ NLG).}
Across evaluation suites spanning multiple tasks, we observe pronounced variation by task type. On NLU-style tasks (often multiple-choice), no configuration is a clear winner across all datasets; performance depends on the base model and the specific benchmark. In contrast, on NLG-style tasks that score free-form generations, models trained on \textbf{Updesh} consistently perform strongly, while remaining competitive (but not dominant) on NLU. This pattern suggests that instruction-following quality and discourse control learned during training transfer more directly to NLG than to choice-based NLU.

\paragraph{Evaluation protocol differences matter.}
Most NLU evaluations compute correctness via likelihood comparisons over \emph{(context, option)} pairs, effectively testing calibrated discrimination among short alternatives. NLG evaluations, by design, require longer generations and measure faithfulness, adequacy, and fluency under open-ended prompting. The divergence in scoring objectives partially explains why a dataset that emphasizes long-form instruction-following (like \textbf{Updesh}) yields larger gains on NLG than on likelihood-based NLU.

We find that \textbf{Bactrian} tends to outperform on NLU-style benchmarks. Two factors may contribute: (i) \emph{format alignment}, as \textbf{Bactrian} contains a larger proportion of MCQ-like or short-form prompts; and (ii) \emph{effective training exposure}, since the dataset is smaller, we matched training steps by repeating it more, increasing the number of MCQ-formatted updates relative to other corpora. Both effects would advantage NLU likelihood tests.

\paragraph{Distribution mismatch between train and test.}
\textbf{Updesh} contains longer-context samples and lacks MCQ-style items; its task composition emphasizes multi-step, generative instruction-following. Many NLU benchmarks, however, are MCQ-heavy and short-context. This \emph{composition shift} (task format, length, and response style) likely depresses relative NLU gains for \textbf{Updesh}-trained models while amplifying NLG gains. In short, models generalize best to evaluation formats that resemble their training distribution.






\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{evaluation_plots/combined_model_trends_by_taxonomy.pdf}
    \caption{Enter Caption}
    \label{fig:placeholder}
\end{figure}


\section{Discussion}


==> macros.tex <==
\newcommand{\VG}[1]{\textit{\textcolor{magenta}{VG: #1}}}
\newcommand{\PAC}[1]{\textit{\textcolor{blue}{PAC: #1}}}
\newcommand{\SA}[1]{\textit{\textcolor{orange}{SA: #1}}}
\newcommand{\SYS}[1]{\textit{\textcolor{teal}{SS: #1}}}
\newcommand{\PK}[1]{\textit{\textcolor{green}{PK: #1}}}

\newcommand{\dsetname}{\textsc{Updesh}\xspace}
\newcommand{\phiBM}{\textsc{Phi4-14B}\xspace}
\newcommand{\llamaBM}{\textsc{Llama-3.1-8B}\xspace}
\newcommand{\llamaIXL}{\textsc{Llama-3.1-405B-Instruct}\xspace}
\newcommand{\llamaIL}{\textsc{Llama-3.3-70B-Instruct}\xspace}
\newcommand{\llamaIM}{\textsc{Llama-3.1-8B-Instruct}\xspace}
\newcommand{\gpto}{\textsc{GPT-4o}\xspace}

\newcommand{\qwenIXL}{\textsc{Qwen3-235B-A22B}\xspace}
\newcommand{\orcaagent}{\textsc{OrcaAgent-Instruct}\xspace}
\newcommand{\lima}{\textsc{LIMA-X}\xspace}
\newcommand{\orcamath}{\textsc{OrcaMath}\xspace}
\newcommand{\aya}{\textsc{Aya-Collection}\xspace}
\newcommand{\bactrian}{\textsc{Bactrian-X}\xspace}
\newcommand{\malpaca}{\textsc{mAlpaca}\xspace}
\newcommand{\alpaca}{\textsc{Alpaca}\xspace}
\newcommand{\indicalign}{\textsc{IndicAlign}\xspace}
\newcommand{\indictrans}{\textsc{IndicTrans2}\xspace}

\newcommand{\phiUp}{\textsc{Phi4-Updesh}\xspace}
\newcommand{\llamaUp}{\textsc{Llama-Updesh}\xspace}

==> tables/downstream_evaluation.tex <==
% % \usepackage{array}
% % \usepackage{multirow}
% % \usepackage{ragged2e}
% % \usepackage{booktabs}


% \begin{table}[ht]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{>{\centering\hspace{0pt}}m{0.112\linewidth}>{\centering\hspace{0pt}}m{0.123\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.094\linewidth}>{\centering\hspace{0pt}}m{0.075\linewidth}>{\centering\hspace{0pt}}m{0.073\linewidth}>{\centering\arraybackslash\hspace{0pt}}m{0.075\linewidth}} 
% \hline\hline
% \textbf{Model}                                   & \textbf{Setting}     & \textbf{MMLU}   & \begin{tabular}[c]{@{}c@{}}\textbf{MMLU }\\\textbf{Indic}\end{tabular} & \textbf{MILU}   & \begin{tabular}[c]{@{}c@{}}\textbf{ARC }\\\textbf{Indic}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{BoolQ }\\\textbf{Indic}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{TriviaQA }\\\textbf{Indic}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Flores }\\\textbf{EnXX}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Flores }\\\textbf{XXEn}\end{tabular} & \textbf{Xsum}   \\ 
% \hline\hline
% \multirow{5}{*}{\Centering{}\textbf{Llama 8B }} & \textbf{Zero Shot}    & 0.2300          & 0.2296                                                                 & 0.2602          & 0.2525                                                                & 0.6204                                                                  & 0.2655                                                                     & 1.00                                                                    & 36.91                                                                   & 0.16            \\
%                                                  & \textbf{Bactrian}    & \textbf{0.634}  & \textbf{0.3679}                                                        & \textbf{0.4220} & 0.2648                                                                &                                                                         & \textbf{0.6630}                                                            & 23.68                                                                   & 46.31                                                                   & 0.2055          \\
%                                                  & \textbf{IndicAlign}  & 0.6044          & 0.3447                                                                 & 0.4192          & 0.2734                                                                &                                                                         & 0.5934                                                                     &                                                                         &                                                                         &                 \\
%                                                  & \textbf{Aya Dataset} & 0.5905          & 0.3268                                                                 & 0.3898          & 0.2810                                                                &                                                                         & 0.5065                                                                     &                                                                         &                                                                         & 0.2433          \\
%                                                  & \textbf{Updesh}      & 0.5135          & 0.3440                                                                 & 0.3742          & \textbf{0.2966}                                                       & \textbf{0.7751}                                                         & 0.4612                                                                     & \textbf{32.63}                                                          & \textbf{46.83}                                                          & \textbf{17.38}  \\ 
% \midrule
%                                                  &                      &                 &                                                                        &                 &                                                                       &                                                                         &                                                                            &                                                                         &                                                                         &                 \\ 
% \midrule
% \multirow{5}{*}{\Centering{}\textbf{Phi4 }}      & \textbf{Zero Shot}    & 0.7781          & 0.4337                                                                 & 0.5194          & 0.2998                                                                & 0.7956                                                                  & 0.6825                                                                     & 23.032                                                                  & 51.38                                                                   & \textbf{11.31}  \\
%                                                  & \textbf{Bactrian}    & \textbf{0.7819} & 0.3990                                                                 & 0.4836          & 0.2939                                                                & 0.7439                                                                  & 0.6729                                                                     & 25.93                                                                   & 47.74                                                                   & 0.31            \\
%                                                  & \textbf{IndicAlign}  & 0.7734          & 0.4526                                                                 & 0.5117          & 0.3247                                                                & 0.7639                                                                  & 0.6235                                                                     & 27.48                                                                   & 1.77                                                                    & 0.27            \\
%                                                  & \textbf{Aya Dataset} & 0.7763          & 0.4507                                                                 & 0.5323          & \textbf{0.3300}                                                       & 0.7261                                                                  & \textbf{0.7180}                                                            & 26.51                                                                   & 7.63                                                                    & 0.36            \\
%                                                  & \textbf{Updesh}      & 0.7762          & \textbf{0.4897}                                                        & \textbf{0.5356} & 0.3207                                                                & \textbf{0.8138}                                                         & 0.6013                                                                     & \textbf{34.57}                                                          & \textbf{53.28}                                                          & 10.21           \\
% \hline\hline
% \end{tabular}
% }
% \end{table}

% Required packages
% \usepackage{array}
% \usepackage{multirow}
% \usepackage{ragged2e}
% \usepackage{booktabs}
% \usepackage{graphicx} % For \resizebox

% \begin{table}
% \centering
% \caption{NLU Task Performance}
% \label{tab:nlu-tasks}
% \begin{tabular}{llccccccccc} 
% \hline\hline
% \textbf{Model}                     & \textbf{Setting}    & \textbf{MMLU}   & \textbf{MMLU Indic} & \textbf{MILU}   & \textbf{ARC Indic} & \textbf{BoolQ Indic} & \textbf{TriviaQA Indic} & \textbf{BeleBele} & \textbf{INCLUDE} & \textbf{GLOBAL MMLU}  \\ 
% \hline\hline
% \multirow{5}{*}{\textbf{Llama 8B}} & \textbf{Zero Shot}  & 0.2300          & 0.2296              & 0.2602          & 0.2525             & 0.6204               & 0.2655                  & 0.2405            & 0.2487           & 0.2301                \\
% & \textbf{Bactrian}   & \textbf{0.634}  & \textbf{0.3679}     & \textbf{0.4220} & 0.2648             & -                    & \textbf{0.6630}         & 0.4145            & 0.3914           & 0.4214                \\
% & \textbf{IndicAlign} & 0.6044          & 0.3447              & 0.4192          & 0.2734             & 0.7114               & 0.5934                  & 0.3209            & 0.3436           & 0.3866                \\
% & \textbf{Aya}        & 0.5905          & 0.3268              & 0.3898          & 0.2810             & 0.7624               & 0.5065                  & 0.4653            & 0.3384           & 0.3681                \\
% & \textbf{Updesh}     & 0.5135          & 0.3440              & 0.3742          & \textbf{0.2966}    & \textbf{0.7751}      & 0.4612                  & \textbf{0.5129}   & 0.3056           & 0.3742                \\ 
% \midrule
% \multirow{5}{*}{\textbf{Phi4}}     & \textbf{Zero Shot}  & 0.7781          & 0.4337              & 0.5194          & 0.2998             & 0.7956               & 0.6825                  & 0.5454            & 0.4545           & 0.5496                \\
% & \textbf{Bactrian}   & \textbf{0.7819} & 0.3990              & 0.4836          & 0.2939             & 0.7439               & 0.6729                  & 0.4831            & 0.4171           & 0.4789                \\
% & \textbf{IndicAlign} & 0.7734          & 0.4526              & 0.5117          & 0.3247             & 0.7639               & 0.6235                  & 0.5167            & 0.4470           & 0.5391                \\
% & \textbf{Aya}        & 0.7763          & 0.4507              & 0.5323          & \textbf{0.3300}    & 0.7261               & \textbf{0.7180}         & 0.6070            & 0.4801           & 0.5347                \\
% & \textbf{Updesh}     & 0.7762          & \textbf{0.4897}     & \textbf{0.5356} & 0.3207             & \textbf{0.8138}      & 0.6013                  & \textbf{0.7441}   & 0.4724           & 0.5746                \\
% \hhline{~==========}
% \end{tabular}
% \end{table}


% \usepackage{multirow}
% \usepackage{booktabs}






% \begin{table}[t]
% \caption{NLU task performance}
% \label{tab:nlu-tasks}

% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llccccccccc} 
% \hline\hline
% \textbf{Model}                     & \textbf{Setting}    & \textbf{MMLU}   & \textbf{MMLU Indic} & \textbf{MILU}   & \textbf{ARC Indic} & \textbf{BoolQ Indic} & \textbf{TriviaQA Indic} & \textbf{BeleBele} & \textbf{INCLUDE} & \textbf{GLOBAL MMLU}  \\ 
% \hline\hline
% \multirow{5}{*}{\textbf{Llama 8B}} & \textbf{Zero Shot}  & 0.2300          & 0.2296              & 0.2602          & 0.2525             & 0.6204               & 0.2655                  & 0.2405            & 0.2487           & 0.2301                \\
%                                    & \textbf{Bactrian}   & \textbf{0.634}  & \textbf{0.3679}     & \textbf{0.4220} & 0.2648             & -                    & \textbf{0.6630}         & 0.4145            & 0.3914           & 0.4214                \\
%                                    & \textbf{IndicAlign} & 0.6044          & 0.3447              & 0.4192          & 0.2734             & 0.7114               & 0.5934                  & 0.3209            & 0.3436           & 0.3866                \\
%                                    & \textbf{Aya}        & 0.5905          & 0.3268              & 0.3898          & 0.2810             & 0.7624               & 0.5065                  & 0.4653            & 0.3384           & 0.3681                \\
%                                    & \textbf{Updesh}     & 0.5135          & 0.3440              & 0.3742          & \textbf{0.2966}    & \textbf{0.7751}      & 0.4612                  & \textbf{0.5129}   & 0.3056           & 0.3742                \\ 
% \midrule
% \multirow{5}{*}{\textbf{Phi4}}     & \textbf{Zero Shot}  & 0.7781          & 0.4337              & 0.5194          & 0.2998             & 0.7956               & 0.6825                  & 0.5454            & 0.4545           & 0.5496                \\
%                                    & \textbf{Bactrian}   & \textbf{0.7819} & 0.3990              & 0.4836          & 0.2939             & 0.7439               & 0.6729                  & 0.4831            & 0.4171           & 0.4789                \\
%                                    & \textbf{IndicAlign} & 0.7734          & 0.4526              & 0.5117          & 0.3247             & 0.7639               & 0.6235                  & 0.5167            & 0.4470           & 0.5391                \\
%                                    & \textbf{Aya}        & 0.7763          & 0.4507              & 0.5323          & \textbf{0.3300}    & 0.7261               & \textbf{0.7180}         & 0.6070            & 0.4801           & 0.5347                \\
%                                    & \textbf{Updesh}     & 0.7762          & \textbf{0.4897}     & \textbf{0.5356} & 0.3207             & \textbf{0.8138}      & 0.6013                  & \textbf{0.7441}   & 0.4724           & 0.5746                \\
% \hline\hline
% \end{tabular}
% }
% \end{center}
% \end{table}

% \begin{table}[t]

% \caption{NLG task performance}
% \label{tab:nlg-tasks}

% \begin{center}
% \small
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{llcccccc} 
% \hline\hline
% \textbf{Model}                     & \textbf{Setting}    & \textbf{Xsum}      & \textbf{Flores EnXX} & \textbf{Flores XXEn} & \textbf{in22-conv-doc} & \textbf{in22-gen} & \textbf{ntrex} \\ 
% \hline\hline
% \multirow{5}{*}{\textbf{Llama 8B}} & \textbf{Zero Shot}  & 0.1621             & 1.0022               & 36.9116              & 0.4461                 & -                  & -              \\
%                                    & \textbf{Bactrian}   & 0.2055             & 23.6897              & 46.3112              & 14.0861                & -                  & -              \\
%                                    & \textbf{IndicAlign} & 9.2603             & 25.1814              & 2.2887               & 10.9765                & -                  & -              \\
%                                    & \textbf{Aya}        & 0.2421             & 22.6022              & 0.5301               & 6.7251                 & -                  & -              \\
%                                    & \textbf{Updesh}     & \textbf{17.3888}  & \textbf{32.6301}    & \textbf{46.8400}    & \textbf{21.2512}      & -                  & -              \\ 
% \midrule
% \multirow{5}{*}{\textbf{Phi4}}     & \textbf{Zero Shot}  & \textbf{11.3197}  & 23.0329              & 51.3888              & 22.7953                & -                  & -              \\
%                                    & \textbf{Bactrian}   & 0.3142             & 25.9317              & 47.7465              & 15.4504                & -                  & -              \\
%                                    & \textbf{IndicAlign} & 0.2742             & 27.4849              & 1.7737               & 13.8207                & -                  & -              \\
%                                    & \textbf{Aya}        & 0.3698             & 26.5106              & 7.6347               & 14.0112                & -                  & -              \\
%                                    & \textbf{Updesh}     & 10.2141            & \textbf{34.5753}    & \textbf{53.2856}    & 18.7371                & -                  & -              \\
% \hline\hline
% \end{tabular}
% }
% \end{center}
% \end{table}





==> tables/tab_results_instfollowing.tex <==
% \begin{table}[!htbp]
% \caption{\textbf{Instruction-following capabilities.} All entries are \emph{accuracy} (higher is better).}
% \centering
% \small
% \begin{tabular}{llcccccccc} 
% \toprule
% \multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Setting}} & \multicolumn{4}{c}{\textbf{mIFEval}} & \multicolumn{4}{c}{\textbf{mIFBench}} \\
% \cmidrule(lr){3-6} \cmidrule(lr){7-10}
% & & \multicolumn{2}{c}{\textbf{Native}} & \multicolumn{2}{c}{\textbf{in English}} & \multicolumn{2}{c}{\textbf{Native}} & \multicolumn{2}{c}{\textbf{in English}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
% & & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} \\
% \midrule
% \multirow{5}{*}{\textbf{Llama}}
% & \textbf{Base} & \textbf{0.24} & \textbf{0.36} & 0.18 & 0.31 & 0.19 & 0.21 & 0.16 & 0.17 \\
% & \textbf{Bactrian} & 0.17 & 0.27 & 0.14 & 0.25 & 0.17 & 0.18 & 0.11 & 0.13 \\
% & \textbf{Indic-Align} & 0.16 & 0.24 & 0.14 & 0.23 & 0.17 & 0.19 & 0.16 & 0.17 \\
% & \textbf{Aya} & 0.13 & 0.22 & 0.11 & 0.21 & \textbf{0.18} & \textbf{0.19} & \textbf{0.18} & \textbf{0.19} \\
% & \textbf{Updesh} & 0.20 & 0.30 & 0.18 & 0.28 & 0.16 & 0.19 & 0.14 & 0.15 \\
% \midrule
% \multirow{5}{*}{\textbf{Phi4}}
% & \textbf{Base} & 0.22 & 0.32 & 0.19 & \textbf{0.30} & 0.14 & 0.16 & 0.13 & 0.14 \\
% & \textbf{Bactrian} & 0.22 & 0.32 & 0.19 & \textbf{0.30} & 0.20 & 0.21 & 0.15 & 0.16 \\
% & \textbf{Indic-Align} & 0.16 & 0.25 & 0.15 & 0.24 & 0.15 & 0.17 & 0.14 & 0.16 \\
% & \textbf{Aya} & 0.15 & 0.25 & 0.14 & 0.24 & 0.20 & 0.21 & \textbf{0.19} & \textbf{0.20} \\
% & \textbf{Updesh} & 0.22 & 0.32 & \textbf{0.19} & 0.29 & \textbf{0.19} & \textbf{0.22} & 0.16 & 0.18 \\
% \bottomrule
% \end{tabular}
% \label{tab:if-capabilities}
% \end{table}



\begin{table*}[!htbp]
\centering
\small
\begin{tabular}{llcccccccc} 
\toprule
\multirow{3}{*}{\textbf{Model}} & \multirow{3}{*}{\textbf{Setting}} & \multicolumn{4}{c}{\textbf{mIFEval}} & \multicolumn{4}{c}{\textbf{mIFBench}} \\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & \multicolumn{2}{c}{\textbf{Native}} & \multicolumn{2}{c}{\textbf{in English}} & \multicolumn{2}{c}{\textbf{Native}} & \multicolumn{2}{c}{\textbf{in English}} \\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} & \textbf{Prompt} & \textbf{Inst.} \\
\midrule
\multirow{5}{*}{\textbf{Llama}}
& \textbf{Base} & \textbf{0.24} & \textbf{0.36} & \textbf{0.18} & \textbf{0.31} & \textbf{0.19} & \textbf{0.21} & 0.16 & 0.17 \\
& \textbf{\bactrian} & 0.17 & 0.27 & 0.14 & 0.25 & 0.17 & 0.18 & 0.11 & 0.13 \\
& \textbf{\indicalign} & 0.16 & 0.24 & 0.14 & 0.23 & 0.17 & 0.19 & 0.16 & 0.17 \\
& \textbf{\aya} & 0.13 & 0.22 & 0.11 & 0.21 & 0.18 & 0.19 & \textbf{0.18} & \textbf{0.19} \\
& \textbf{\dsetname} & 0.20 & 0.30 & \textbf{0.18} & 0.28 & 0.16 & 0.19 & 0.14 & 0.15 \\
\midrule
\multirow{5}{*}{\textbf{Phi4}}
& \textbf{Base} & \textbf{0.22} & \textbf{0.32} & \textbf{0.19} & \textbf{0.30} & 0.14 & 0.16 & 0.13 & 0.14 \\
& \textbf{bactrian} & \textbf{0.22} & \textbf{0.32} & \textbf{0.19} & \textbf{0.30} & \textbf{0.20} & 0.21 & 0.15 & 0.16 \\
& \textbf{\indicalign} & 0.16 & 0.25 & 0.15 & 0.24 & 0.15 & 0.17 & 0.14 & 0.16 \\
& \textbf{\aya} & 0.15 & 0.25 & 0.14 & 0.24 & \textbf{0.20} & 0.21 & \textbf{0.19} & \textbf{0.20} \\
& \textbf{\dsetname} & \textbf{0.22} & \textbf{0.32} & \textbf{0.19} & 0.29 & 0.19 & \textbf{0.22} & 0.16 & 0.18 \\
\bottomrule
\end{tabular}
\caption{Instruction-following capabilities. All entries are \emph{accuracy} (higher is better).}
\label{tab:if-capabilities}
\end{table*}

% \VG{what is base here? I assume it is the instruct variant? - No base}
